Spectral-GS: Taming 3D Gaussian Splatting with Spectral Entropy

Recently, 3D Gaussian Splatting (3D-GS) has achieved impressive results in novel view synthesis, demonstrating high fidelity and efficiency. However, it easily exhibits needle-like artifacts, especially when increasing the sampling rate. Mip-Splatting tries to remove these artifacts with a 3D smoothing filter for frequency constraints and a 2D Mip filter for approximated supersampling. Unfortunately, it tends to produce over-blurred results, and sometimes needle-like Gaussians still persist. Our spectral analysis of the covariance matrix during optimization and densification reveals that current 3D-GS lacks shape awareness, relying instead on spectral radius and view positional gradients to determine splitting. As a result, needle-like Gaussians with small positional gradients and low spectral entropy fail to split and overfit high-frequency details. Furthermore, both the filters used in 3D-GS and Mip-Splatting reduce the spectral entropy and increase the condition number during zooming in to synthesize novel view, causing view inconsistencies and more pronounced artifacts. Our Spectral-GS, based on spectral analysis, introduces 3D shape-aware splitting and 2D view-consistent filtering strategies, effectively addressing these issues, enhancing 3D-GS's capability to represent high-frequency details without noticeable artifacts, and achieving high-quality photorealistic rendering.

==> sec/tab_and_fig/issue_split_img.tex <==

\begin{figure}[!t]

\includegraphics[width=1\linewidth]{figures/issue_split_img.pdf}
\caption{We visualize the spectral entropy maps of 3D Gaussians after optimization. This clearly demonstrates the spectral entropy distribution and the degree of anisotropy of 3D Gaussians that influence needle-like artifacts in 3D-GS ~\cite{kerbl20233d} and Mip-Splatting~\cite{mip_gs}.  Middle the
corresponding rendered images.} 
\label{fig:issue_split_img}
% \vspace{-0.2cm}
\end{figure}


==> sec/tab_and_fig/lod.tex <==

\begin{figure}[t]

\includegraphics[width=1\linewidth]{figures/lod.pdf}
\caption{} 
\label{fig:lod}

\end{figure}


==> sec/tab_and_fig/reg_img.tex <==

\begin{figure}[t]

\includegraphics[width=1\linewidth]{figures/reg_img.pdf}
\caption{We show the results of introducing a regularization term $\mathcal{L}_{\boldsymbol{\Sigma}}$ into the loss function.} 
\label{fig:reg_img}

\end{figure}

